Limits on contact interactions and leptoquarks at HERA

High-precision HERA data corresponding to a luminosity of around 1 fb$^{-1}$ have been used in the framework of $eeqq$ contact interactions (CI) to set limits on possible high-energy contributions beyond the Standard Model to electron-quark scattering. Measurements of the inclusive deep inelastic cross sections in neutral and charged current $ep$ scattering were considered. The analysis of the $ep$ data has been based on simultaneous fits of parton distribution functions including contributions of CI couplings to $ep$ scattering. Several general CI models and scenarios with heavy leptoquarks were considered. Improvements in the description of the inclusive HERA data were obtained for a few models. Since a statistically significant deviation from the Standard Model cannot be established, limits in the TeV range were set on all models considered.

==> ci_paper-cit.tex <==
%==============================================================================
% Some definitions of citations
%==============================================================================
%------------------------------------------------------------------------------
% -> CTD
%------------------------------------------------------------------------------
\def\citeCTD{{\cite{%
nim:a279:290,*npps:b32:181,*nim:a338:254%
}}\xspace}
%------------------------------------------------------------------------------
% -> MVD
%------------------------------------------------------------------------------
\def\citeMVD{{\cite{%
nim:a581:656%
}}\xspace}
%------------------------------------------------------------------------------
% -> STT
%------------------------------------------------------------------------------
\def\citeSTT{{\cite{%
nim:a535:191%
}}\xspace}
%------------------------------------------------------------------------------
% -> CAL
%------------------------------------------------------------------------------
\def\citeCAL{{\cite{%
nim:a309:77,*nim:a309:101,*nim:a321:356,*nim:a336:23%
}}\xspace}
%------------------------------------------------------------------------------
% -> HES
%------------------------------------------------------------------------------
\def\citeHES{{\cite{%
nim:a277:176%
}}\xspace}
%------------------------------------------------------------------------------
% -> 6mT
%------------------------------------------------------------------------------
\def\citeSixmT{{\cite{%
thesis:gosau:2007%
}}\xspace}
%------------------------------------------------------------------------------
% -> BAC
%------------------------------------------------------------------------------
\def\citeBAC{{\cite{%
nim:a300:480%
}}\xspace}
%------------------------------------------------------------------------------
% -> LUMI
%------------------------------------------------------------------------------
\def\citePCAL{{\cite{%
desy-92-066,*zfp:c63:391,*acpp:b32:2025%
}}\xspace}
\def\citeSPECTRO{{\cite{%
nim:a565:572%
}}\xspace}

